Exploring Cluster Analysis in Nelore Cattle Visual Score Attribution

Assessing the biotype of cattle through human visual inspection is a very common and important practice in precision cattle breeding. This paper presents the results of a correlation analysis between scores produced by humans for Nelore cattle and a variety of measurements that can be derived from images or other instruments. It also presents a study using the k-means algorithm to generate new ways of clustering a batch of cattle using the measurements that most correlate with the animal's body weight and visual scores.

==> ajustes.tex <==
\newcommand{\nomeEditor}{Spyros Fountas}
\newcommand{\nomeArtigo}{Exploring Cluster Analysis in Nelore Cattle Visual Score Attribution}
\newcommand{\nomeRevista}{Smart Agricultural Technology}

